Simple Stochastic Games with Almost-Sure Energy-Parity Objectives are in NP and coNP

We study stochastic games with energy-parity objectives, which combine quantitative rewards with a qualitative $\omega$-regular condition: The maximizer aims to avoid running out of energy while simultaneously satisfying a parity condition. We show that the corresponding almost-sure problem, i.e., checking whether there exists a maximizer strategy that achieves the energy-parity objective with probability $1$ when starting at a given energy level $k$, is decidable and in $NP \cap coNP$. The same holds for checking if such a $k$ exists and if a given $k$ is minimal.

==> app.6.tex <==
\subsection{$\Gain$ is in $\coNP$} 
\label{app:gain-coNP}
\coNPgain*
\begin{proof}
By \cref{lem:gain:min-MD}, it suffices to show \coNP\ membership only for the MDP case,
as a witnessing MD strategy for minimizer can be guessed as part of the certificate. 
To do this, we can use \cite[Lemma~26]{MSTW2017}, which says that we can compute
$\LVal{s} \eqdef \sup_{k}\Val{s}{\EN{k}\cap\Parity}$.

The correctness of this reduction relies on 
the fact that 
$$\LVal{s} = \Val{s}{\LimInf{>-\infty}\cap\Parity} = \Val{s}{\Gain}$$
To see this,
notice that for every fixed $k\in\N$ we have
$$\Val{s}{\EN{k}\cap\Parity}
\le
\Val{s}{\LimInf{>-\infty}\cap\Parity}.$$
Since the limit-payoff-and-parity objective is shift-invariant, by \cite{GH2010} there exist optimal strategies $\sigma,\tau$
such that
$\Val{s}{\LimInf{>-\infty}\cap\Parity}
=
\Prob[\sigma,\tau]{s}(\LimInf{>-\infty}\cap\Parity)
$.
This is less or equal to $\LVal{s}$ by \cref{lem:gain:min-MD}, since the
guessed minimizer MD strategy is optimal.
\end{proof}

\subsection{$\sys{G} \to \sys{G}_1 \to \sys{G}_2 \to \sys{G}_3$ constructions}
\label{app:gain-NP}

Before we can proceed with the technical details of the
$\sys{G} \to \sys{G}_1 \to \sys{G}_2 \to \sys{G}_3$ constructions,
we first need to introduce the following standard definitions.

\begin{definition}
    Let $\sys{M}=\sys{G}[\tau]$ be an MDP induced by game $\sys{G}\eqdef(V=(\VMax,\VMin,\VRan), E, \prob)$ and an MD strategy $\tau$ for minimizer.
    An \emph{end-component} is a strongly connected set of states $C \subseteq V$ such that, for every state $v\in C$,
    if $v \in \VMax$ then some successor $v'$ of $v$ is in $C$, and
    if $v \in \VRan\cup\VMin$ then all successors $v'$ of $v$ are in $C$.
    A \emph{leaf-component} is an end-component of a Markov chain $\sys{G}[\sigma,\tau]$.
    
    A leaf-component is \emph{\safe} if the dominating priority is even and it satisfies the storage condition $\bigcup_{k\ge 0}{\ES{k}}$, and 
    \emph{\positive} if its mean-payoff is positive.
    
    An end-component $C$ of $\sys{G}[\tau]$ is \emph{\awesome} if (1) the dominating priority of $C$
    (the smallest priority of any state in $C$) is even and $C$ contains a \positive leaf-component
    \emph{or} (2)
    there is an MD strategy $\sigma$ for the maximizer, such that $C$ is a \safe leaf-component in $\sys{G}[\sigma,\tau]$. 
\end{definition}

Note that any end-component that satisfies a.s.~$\Gain$ is \awesome, which justifies its name. This is because either (1) holds, or else maximizer can reach again and again a state with a dominating even priority without the need to pump up the energy level first for which an MD strategy suffices, so (2) would hold then.

\subsubsection{Blow-up Construction ($\sys{G} \to \sys{G}_1)$.}
\label{app:g-to-g1}
\input{sec.gain.NP.blowup}
\input{app.6.NP.blowup}

\subsubsection{Trade-in Construction ($\sys{G}_1 \to \sys{G}_2)$.}
\label{app:g1-to-g2}
\label{sec:gain.NP.tradein}
\input{sec.gain.NP.tradein}
\input{app.6.NP.tradein}

\subsubsection{Concise Witnesses Construction ($\sys{G}_2 \to \sys{G}_3$).}
\input{sec.gain.NP.concise}
\input{ex.NP}



==> app.correctness.tex <==

Before we prove \cref{thm:correctness},
we will collect the remaining technical claims
about $\Gain$, $\Bailout$, and reachability objectives.
Most notably, as \cref{lem:gain-value},
we show that if maximizer can almost surely win $\Gain$ in a SSG,
then he can do so using a FD strategy which moreover satisfies an energy-parity objective
with strictly positive (and lower-bounded) probability.
This is shown in part based on \cref{lem:FD-strategy} applied to the $\Gain$ objective.
We will also need the following fact about reachability objectives in finite MDPs.

\begin{lemma}[{\cite[Lemma~3.9]{BBEK:IC2013}}]\label{BBEK:IC2013:Lemma3.9}
Let $\?M$ be a finite MDP and $T \eqdef \{s'\ |\ \Val{s'}{\LimInf{=-\infty}}=1\}$
and ${\it Reach}_T$ the set of runs visiting $T$.
One can compute a rational constant $c< 1$
and an integer $h \ge 0$ such that for all states $s$ and 
$i \ge h$ we have
$
\forall \tau.\, \Prob[\tau]{s}(\overline{\EN{i}} \cap \overline{{\it Reach}_T}) \le \frac{c^i}{1-c}
$.
\end{lemma}


\begin{lemma}\label{lem:gain-value}
Consider a finite SSG $\?G=(V,E,\prob)$ 
where $\Gain$ holds a.s.\ for every state $s\in V$.
Then, for every $\delta \in [0,1)$ and $s \in V$, there exists a
$\hat{k} \in \N$
and an FD strategy $\hat{\sigma}$
s.t. 
\begin{enumerate}
\item
$\forall \tau.\, \Prob[\hat{\sigma},\tau]{s}(\Gain)=1$, and \label{lem:gain-value-ad1}
\item
$\forall \tau.\, \Prob[\hat{\sigma},\tau]{s}(\EN{\hat{k}} \cap \Parity) \ge \delta$.
\label{lem:gain-value-ad2}
\end{enumerate}
\end{lemma}
\begin{proof}
Fix a $\delta \in [0,1)$ and a state $s \in V$.
Both $\LimInf{=-\infty}$, as well as $\Parity$ objectives are 
\emph{shift-invariant} and \emph{submixing},
and therefore also the union has both these
properties.
It follows
that $\overline{\Gain} = \overline{\LimInf{>-\infty}\cap\Parity} = \LimInf{=-\infty}\cup\overline{\Parity}$
is both shift-invariant and submixing, since the complement of a parity
objective is also a parity objective.
By \cref{lem:MDP-FD-strategy} and \cref{lem:FD-strategy}, there exists an almost-sure winning FD
strategy $\hat{\sigma}$ for maximizer for the objective $\Gain$ %
from $s$, 
i.e., 
$\forall \tau.\, \Prob[\hat{\sigma},\tau]{s}(\Gain)=1$,
thus yielding \cref{lem:gain-value-ad1}.

Let $\?M$ be the MDP obtained from $\?G$ by fixing the strategy
$\hat{\sigma}$ for maximizer from $s$.
Since $\?G$ is finite and $\hat{\sigma}$ is FD, also $\?M$ is finite.  
In $\?M$ we have
$\forall \tau.\, \Prob[\tau]{s}(\Gain)=1$.
In particular, in $\?M$, the set $T \eqdef \{s'\ |\ \Val{s'}{\LimInf{=-\infty}}=1\}$
is not reachable, i.e., 
$\forall \tau.\, \Prob[\tau]{s}({\it Reach}_T)=0$.

By \cref{BBEK:IC2013:Lemma3.9}, in $\?M$
there exists a horizon $h \in\N$ and a constant $c <1$ such that for all $i \ge h$ we have
$\forall \tau.\, \Prob[\tau]{s}(\overline{\EN{i}} \cap \overline{{\it Reach}_T}) \le \frac{c^i}{1-c}$.
Since $T$ cannot be reached in $\?M$, the condition $\overline{{\it Reach}_T}$ evaluates 
to ${\it true}$ and we have
$\forall \tau.\, \Prob[\tau]{s}(\EN{i}) \ge 1-\frac{c^i}{1-c}$.
Since $c<1$ and $\delta<1$, we can pick a sufficiently large $\hat{k} \ge h$ such that 
$1-\frac{c^{\hat{k}}}{1-c} \ge \delta$ and obtain
$\forall \tau.\, \Prob[\tau]{s}(\EN{\hat{k}}) \ge \delta$ in $\?M$.
Moreover, the above property 
$\forall \tau.\, \Prob[\tau]{s}(\Gain)=1$
in particular implies 
$\forall \tau.\, \Prob[\tau]{s}(\Parity)=1$.
Thus we obtain
$\forall \tau.\, \Prob[\tau]{s}(\EN{\hat{k}} \cap \Parity) \ge \delta$ in $\?M$.

Back in the SSG $\?G$, we have
$\forall \tau.\, \Prob[\hat{\sigma},\tau]{s}(\EN{\hat{k}} \cap \Parity) \ge \delta$
as required for \cref{lem:gain-value-ad2}.
\end{proof}



\begin{lemma}\label{lem:enpar-bailout}
  $\EN{k} \cap \Parity \subseteq \kBailout$.
\end{lemma}
\begin{proof}
Let $\rho$ be a run in $\EN{k} \cap \Parity$.
There are two cases. In the first case we have $\rho \in \cup_{l} \ES{k,l}\cap\Parity$ and thus
directly $\rho \in \kBailout$.
Otherwise, $\rho \notin \cup_{l} \ES{k,l}\cap\Parity$.
Since $\rho \in \Parity$, we must have $\rho \notin \cup_{l} \ES{k,l}$.
Since $\rho \in \EN{k}$, it follows that $\rho$ does not
satisfy the $l$-storage condition for any $l \in \N$.
So, for every $l \in \N$, there exists an infix $\rho'$ of $\rho$ 
s.t.\ $l + \cost(\rho') < 0$.
Let $\rho''$ be the prefix of $\rho$ before $\rho'$.
Since $\rho \in \EN{k}$ we have $k + \cost(\rho''\rho') \ge 0$
and thus $\cost(\rho'') \ge -k - \cost(\rho') > -k + l$.
To summarize, if $\rho \notin \cup_{l} \ES{k,l}\cap\Parity$
then, for every $l$, it has a prefix $\rho''$ with
$\cost(\rho'') > -k + l$. Thus
$\rho \in \LimSup{=\infty}$.
Thus $\rho \in \kBailout$.
\end{proof}

We now define $W'$ as the set of states that are almost-sure winning for
energy-parity with some sufficiently high initial energy level.
($W'$ is also called the winning set for the unknown initial credit problem.) 
It is used in the proof of the following lemmas and \cref{thm:correctness}.

\begin{definition}\label{def:Wprime}
$W' \eqdef \bigcup_{k} \AS{\EN{k} \cap \Parity}$.
\end{definition}

\begin{lemma}\label{lem:connect-aspar-gain-bailout}
\
\begin{enumerate}
\item\label{lem:connect-aspar-gain-bailout-1}
$\AS{\EN{k} \cap \Parity} \subseteq \AS{\Gain \cap \always W'}$
\item\label{lem:connect-aspar-gain-bailout-2}
$\AS{\EN{k} \cap \Parity} \subseteq \AS{\kBailout \cap \always W'}$
\end{enumerate}
\end{lemma}
\begin{proof}
Let $s \in \AS{\EN{k} \cap \Parity}$ and
$\sigma$ a strategy that witnesses this property.
Except for a null-set, all runs
$\rho = se_0s_1e_1\ldots e_{n-1}s_n \dots$ from $s$ induced by $\sigma$ satisfy
$\EN{k} \cap \Parity$. 

Let $\rho' = se_0s_1e_1\ldots s_m$ be a finite prefix of $\rho$.
For every $n \ge 0$ we have
$k+\sum_{i=0}^{n-1} \cost(e_i) \ge 0$, since $\rho \in \EN{k}$.
In particular this holds for all $n \ge m$.
So, for every $n \ge m$, we have 
$k+\sum_{i=0}^{m-1} \cost(e_i) + \sum_{i=m}^{n-1} \cost(e_i) \ge 0$.
Therefore $s_m \in \AS{\EN{k'} \cap \Parity}$, where
$k' = k+\sum_{i=0}^{m-1} \cost(e_i)$, as witnessed by playing $\sigma$
with history $se_0s_1e_1\ldots s_m$ from $s_m$.
Thus $s_m \in \bigcup_{k} \AS{\EN{k} \cap \Parity} = W'$, i.e., 
almost all $\sigma$-induced runs $\rho$ satisfy $\always W'$.

Towards \cref{lem:connect-aspar-gain-bailout-1},
we have $\EN{k} \subseteq \LimInf{>-\infty}$ and
thus $\EN{k} \cap \Parity \subseteq \LimInf{>-\infty}\cap\Parity = \Gain$.
Therefore $\sigma$ witnesses
$s \in \AS{\Gain \cap \always W'}$.

Towards \cref{lem:connect-aspar-gain-bailout-2},
we have $\EN{k} \cap \Parity \subseteq \kBailout$
by \cref{lem:enpar-bailout}.
Thus $\sigma$ witnesses $s \in \AS{\kBailout \cap \always W'}$.
\end{proof}

\begin{lemma}\label{claim1}
$W' \subseteq W$.
\end{lemma}
\begin{proof}
It suffices to show that $W'$ satisfies the monotone condition imposed on
$W$ (cf. \cref{def:W}), since $W$ is defined as the largest set satisfying this condition.

Let $s \in W' = \bigcup_{k} \AS{\EN{k} \cap \Parity}$.
Then $s \in \AS{\EN{\hat{k}} \cap \Parity}$ for some fixed $\hat{k}$.
By \cref{lem:connect-aspar-gain-bailout}(1) we have
$s \in \AS{\Gain \cap \always W'}$.
By \cref{lem:connect-aspar-gain-bailout}(2) we have
$s \in \AS{\hat{k}\text{-}\Bailout \cap \always W'}
\subseteq
\bigcup_{k}\AS{\kBailout \cap \always W'}$.
\end{proof}


\thmCorrectness*
\begin{proof} %
Towards the $\subseteq$ inclusion,
we have
\[
\AS{\EN{k} \cap \Parity}
\subseteq
\AS{\kBailout \cap \always W'}
\subseteq
\AS{\kBailout \cap \always W}
\]
by \cref{lem:connect-aspar-gain-bailout}(2)
and
\cref{claim1}.

Towards the $\supseteq$ inclusion, let 
$s \in \AS{\kBailout \cap \always W}$. We show that 
$s \in \AS{\EN{k} \cap \Parity}$.
Let $\sigma_1$ be a strategy that witnesses that $s \in \AS{\kBailout \cap \always W}$.
We now consider the modified SSG $\?G' = (W,E,\prob)$ with the state set
restricted to $W$. In particular, $s \in W$ and 
$\sigma_1$ witnesses $s \in \AS{\kBailout}$ in $\?G'$.
We now construct a strategy $\sigma$ that witnesses 
$s \in \AS{\EN{k} \cap \Parity}$ in $\?G'$, and thus also in $\?G$.
The strategy $\sigma$ will use infinite memory to keep track of the
current energy level of the run.

Apart from $\sigma_1$, we require several more strategies as building blocks
for the construction of $\sigma$.

First, in $\?G$ we had $\forall s' \in W.\, s' \in \AS{\Gain \cap \always W}$, 
and thus in $\?G'$ we have $\forall s' \in W.\, s' \in \AS{\Gain}$.
For every $s' \in W$ we instantiate \cref{lem:gain-value} for $\?G'$ with
$\delta = 1/2$ and obtain a number $\hat{k}_{s'}$ and a strategy
$\hat{\sigma}_{s'}$
with
\begin{enumerate}
\item
$\forall \tau.\, \Prob[\hat{\sigma}_{s'},\tau]{s'}(\Gain)=1$, and \label{thm:correctness-ad1}
\item
$\forall \tau.\, \Prob[\hat{\sigma}_{s'},\tau]{s'}(\EN{\hat{k}_{s'}} \cap \Parity) \ge 1/2$.
\label{thm:correctness-ad2}
\end{enumerate}
Let $k_1 \eqdef \max\{\hat{k}_{s'}\ |\ s' \in W\}$.
The strategies $\hat{\sigma}_{s'}$ are called \emph{gain strategies}.

Second, by the finiteness of $V$, there is a minimal number
$k_2$ such that $\bigcup_k \AS{\kBailout \cap \always W} = \bigcup_{k \le k_2}
\AS{\kBailout \cap \always W}$ in $\?G$.
Therefore, in $\?G'$ we have that
$$W \subseteq \bigcup_k \AS{\kBailout} = \bigcup_{k \le k_2}
\AS{\kBailout} = \AS{k_2\text{-}\Bailout}.$$
Thus in $\?G'$ for every $s' \in W$ there exists a strategy
$\tilde{\sigma}_{s'}$ with
$\forall \tau.\, \Prob[\tilde{\sigma}_{s'},\tau]{s'}(k_2\text{-}\Bailout)
= 1$.
The strategies $\tilde{\sigma}_{s'}$ are called \emph{bailout strategies}.
Let $k' \eqdef k_1 + k_2 - k +1$. We now define the strategy $\sigma$.
\begin{description}
\item[Start:] 
First $\sigma$ plays like $\sigma_1$ from $s$. 
Since $\sigma_1$ witnesses $s \in \AS{\kBailout}$ 
against every minimizer strategy $\tau$, almost all induced runs
$\rho = s e_0s_1e_1\ldots$ satisfy either
\begin{description}
\item[(A)] $(\cup_{l}\ES{k,l} \cap \Parity)$, or
\item[(B)] $(\EN{k} \cap \LimSup{=\infty})$.
\end{description}
Almost all runs $\rho$ of the latter type (B) (and potentially also some runs of type
(A)) satisfy $\EN{k}$ and $\sum_{i=0}^l\cost(e_i) \ge k'$ eventually for some
$l$. 
If we observe $\sum_{i=0}^l\cost(e_i) \ge k'$ for some prefix 
$s e_0s_1e_1\ldots e_l s'$ of the run $\rho$ 
then our strategy $\sigma$ plays from $s'$ as
described in the {\bf Gain} part below.
Otherwise, if we never observe this condition, then our run $\rho$
is of type (A) and $\sigma$ continues playing like $\sigma_1$.
Since property (A) implies $(\EN{k} \cap \Parity)$, this is sufficient.
\item[Gain:]
In this case we are in the situation where we have reached 
some state $s'$ after some finite prefix $\rho'$ of the run, where
$\cost(\rho') \ge k'$. Our strategy $\sigma$ now 
plays like the gain strategy $\hat{\sigma}_{s'}$, as long as
$\cost(\rho') \ge k'-k_1$ holds for the current prefix $\rho'$ of the run.
By \cref{thm:correctness-ad2}, this will satisfy 
$\forall \tau.\, \Prob[\hat{\sigma}_{s'},\tau]{s'}(\EN{\hat{k}_{s'}} \cap
\Parity) \ge 1/2$ and thus 
$\forall \tau.\, \Prob[\hat{\sigma}_{s'},\tau]{s'}(\EN{k_1} \cap \Parity) \ge 1/2$.
It follows that with probability $\ge 1/2$ we will keep playing
$\hat{\sigma}_{s'}$ forever and satisfy $\Parity$ and always $\cost(\rho') \ge k'-k_1$
and thus $\EN{k}$, since $k + \cost(\rho') \ge k+k'-k_1 = k_2 + 1\ge 0$.

Otherwise, if eventually $\cost(\rho') = k'-k_1 -1$ then we have 
$k + \cost(\rho') = k_2$. In this case (which happens with probability $<1/2$)
we continue playing as described in the {\bf Bailout} part below.
\item[Bailout:]\label{item:sigma:bailout}
In this case we are in the situation where we have reached 
some state $s'' \in W$ after some finite prefix $\rho'$ of the run, where
$k+\cost(\rho') = k_2$. 
Since $s'' \in W$, we can now let our strategy $\sigma$ 
play like the bailout strategy $\tilde{\sigma}_{s''}$ and obtain
$\forall \tau.\,
\Prob[\tilde{\sigma}_{s''},\tau]{s''}(k_2\text{-}\Bailout) = 1$.
Thus almost all induced runs $\rho'' = s'' e_0s_1e_1\ldots$ from $s''$ 
satisfy either
\begin{description}
\item[(A)] $(\cup_{l}\ES{k_2,l} \cap \Parity)$, or
\item[(B)] $(\EN{k_2} \cap \LimSup{=\infty})$.
\end{description}
As long as $\cost(\rho') < k'$ holds for the current prefix $\rho'$ of the run, we
keep playing $\tilde{\sigma}_{s''}$. 
Otherwise, if eventually $\cost(\rho') \geq k'$ holds, then we switch back to playing
the {\bf Gain} strategy above.
All the runs that never switch back to playing
the {\bf Gain} strategy must be of type (A) and thus satisfy $\Parity$.
Since we have 
$k_2\text{-}\Bailout \subseteq \EN{k_2}$, it follows that,
for every prefix $\rho''$ of the run from $s''$, according to $\tilde{\sigma}_{s''}$
we have $k_2 + \cost(\rho'') \ge 0$.
Thus, for every prefix $\rho'''$ of $\rho$, we have
$k + \cost(\rho''') = k + \cost(\rho') + \cost(\rho'') = k_2 + \cost(\rho'') \ge 0$.
Therefore, the $\EN{k}$ objective is satisfied by all runs.
\end{description}
As shown above, almost all runs induced by $\sigma$ that eventually stop switching between the three modes
satisfy $\EN{k} \cap \Parity$.
Switching from Gain/Bailout to Start is impossible, but switching from Gain to
Bailout and back is possible. However, the set of runs that infinitely often
switch between Gain and Bailout is a null-set, because the probability of
switching from Gain to Bailout is $\le 1/2$.
Thus, $\sigma$ witnesses $s \in \AS{\EN{k} \cap \Parity}$. 
\end{proof}


\begin{remark}\label{rem:WvsWprime}
It follows from the results above that $W' = W$.
The $\subseteq$ inclusion holds by \cref{claim1}.
For the reverse inclusion we have
\begin{align*}
W &\subseteq  \bigcup_{k}\AS{\kBailout \cap \always W} & \text{by \cref{def:W}}\\
  &=          \bigcup_{k}\AS{\EN{k} \cap \Parity}      & \text{by \cref{thm:correctness}}\\
  &=          W'                                      & \text{by \cref{def:Wprime}}
\end{align*}
\end{remark}



==> sec.intro.old.tex <==
\emph{Simple stochastic games} (SSGs), also called \emph{competitive Markov decision
processes} \cite{Filar_Vrieze:book},
or \emph{$2\frac{1}{2}$-player games} \cite{CJH2004,CJH2003}
are turn-based games of perfect information played on finite graphs.
Each state is either random or belongs to one of the players (maximizer or minimizer).
A play is an infinite path where the next state is chosen by the player who owns the current one,
or according to predefined distribution, in the case of random states.
The maximizer (resp.\ minimizer) tries to maximize (resp.\ minimize)
the expected value of some objective function. %
The maximizer can be seen as a controller trying to ensure an objective in the
face of both known random failure modes (encoded by the random states) and
an unknown or hostile environment (encoded by the minimizer player).

We consider the \emph{energy-parity} objective,
which combines a quantitative (total reward)
with a qualitative ($\omega$-regular) correctness condition.
Numeric rewards are assigned to transitions, and priorities (encoded by bounded
numbers) are assigned to states. This allows to
define quantitative conditions (expressed via the rewards on edges)
and qualitative conditions (expressed via the sequence
of observed priorities).
The \emph{energy-parity} objective is a conjunction of
(1) the energy condition, which asks that the total reward (the system's ``energy level'')
remains non-negative,
and (2) the parity condition, which
asks that the minimal priority that appears infinitely often on the run is even.
Such objectives are very expressive, since the total reward is not
bounded a-priori and parity conditions subsume all simpler $\omega$-regular
objectives like B\"uchi, co-B\"uchi, safety and reachability.
The energy-parity objective is Borel and therefore weakly determined,
meaning that it has a well-defined ($\inf\sup$) value for every game \cite{M1998,Maitra-Sudderth:2003}.
Moreover, the almost-sure energy-parity
objective (asking to win with probability $1$)
is even strongly determined \cite{KMSW2017}: either maximizer has a
strategy to enforce the condition with probability $1$ or minimizer has a
strategy to prevent this.

\input{ex.two-ways}


\mypar{Previous work.}
Non-stochastic energy-parity games have been studied in \cite{CD2010}. They
can be solved in $\NP \cap \coNP$
and maximizer strategies require only
finite (but exponential) memory, a property that also allowed to
show P-time inter-reducibility with mean-payoff parity games.
More recently they were also shown to be solvable in pseudo-quasi-polynomial time \cite{daviaud2018pseudo}.
Related results on non-stochastic games (e.g., mean-payoff parity) are
summarized in \cite{chatterjee2011games}. %

Most existing work
on combined objectives
for stochastic systems, e.g.~\cite{CD2011,chatterjee2011games,BKN2016,MSTW2017},
is restricted to
Markov decision processes (MDPs; aka $1\frac{1}{2}$-player games).
Almost-sure energy-parity objectives for MDPs were first considered in
\cite{CD2011,chatterjee2011games}, %
where a direct reduction to ordinary energy games was proposed.
This reduction relies on the assumption
that maximizer can win using finite memory if at all.
Unfortunately, this assumption does not necessarily hold:
it was shown in \cite{MSTW2017} that an almost sure winning strategy
for energy-parity in finite MDPs may require infinite memory.
Nevertheless, it was possible to recover the original result,
that deciding the existence of a.s.~winning strategies is
in $\NP \cap \coNP$ (and pseudo-polynomial time),
by showing that
the existence of an a.s.~winning strategy
can be witnessed by the existence of two compatible, and finite-memory, winning strategies for two simpler
objectives.
We generalize this approach from MDPs to full stochastic games.

Stochastic mean-payoff parity games were studied in \cite{CDGQ:2014}, where it was shown that
they can be solved in $\NP \cap \coNP$. However, this does not imply a solution for
stochastic energy-parity games, since, unlike in the non-stochastic
case \cite{CD2010},
there is no known reduction from energy-parity to mean-payoff parity
in stochastic games. (The reduction in \cite{CD2010} relies on the fact that
maximizer has a winning finite-memory strategy for energy-parity, which does
not generally hold for stochastic games or MDPs; see above.)

A related model are the 1-counter MDPs (and stochastic games) studied in
\cite{BBEKW2010,BBE2010,BBEK:IC2013}, since the value of the counter can be interpreted as
the stored energy. These papers consider the objective of reaching counter value
zero (which is dual to the energy objective of staying above zero), thus the roles
of minimizer and maximizer are swapped. However, unlike in this paper,
these works do not combine termination objectives with 
extra parity conditions.

\mypar{Our contributions.}
We consider stochastic games with energy-parity winning conditions and show that deciding whether
maximizer can win almost-surely for a given initial energy level $k$ 
is in $\NP \cap \coNP$. We show the same for checking if such $k$ exists at all and 
checking if a given $k$ is the smallest possible for which this holds.
The proofs are considerably harder than the corresponding result for MDPs
\cite{MSTW2017} (on which they are partly based), because the attainable mean-payoff value
is no longer a valid criterion in the analysis (via combinations of sub-objectives).
E.g., even though the stored energy
might be inexorably drifting towards $+\infty$ (resp.\ $-\infty$), the mean-payoff value
might still be zero because the minimizer (resp.\ maximizer) can
delay payoffs for longer and longer (though not indefinitely, due to the
parity condition). Moreover, the minimizer might be able to
choose between different ways of losing and never commit to any particular way
after any finite prefix of the play (see \cref{ex:two-ways}).

Our proof characterizes almost-sure energy-parity via a recursive combination of complex
sub-objectives called \emph{Gain} and \emph{Bailout}, which can each eventually be solved in
$\NP \cap \coNP$.

Our proof of the \coNP\ membership is based on a result 
on the strategy complexity of a natural class of objectives,
which is of independent interest.
We show 
(cf.~\cref{lem:FD-strategy}; based on previous work in \cite{GK2014})
that, if an objective $\?O$ is such that its complement %
is both shift-invariant and submixing,
and that every MDP admits optimal finite-memory
deterministic maximizer strategies for $\?O$, then the same is true in
turn-based stochastic games.


